Accelerating Electrostatics-based Global Placement with Enhanced FFT Computation

Global placement is essential for high-quality and efficient circuit placement for complex modern VLSI designs. Recent advancements, such as electrostatics-based analytic placement, have improved scalability and solution quality. This work demonstrates that using an accelerated FFT technique, AccFFT, for electric field computation significantly reduces runtime. Experimental results on standard benchmarks show significant improvements when incorporated into the ePlace-MS and Pplace-MS algorithms, e.g., a 5.78x speedup in FFT computation and a 32% total runtime improvement against ePlace-MS, with 1.0% reduction of scaled half-perimeter wirelength after detailed placement.

==> tables/tbl-benchmarks.tex <==
\begin{table}[t]
   \centering
   \caption{The MMS benchmark suite~\cite{MMS}}
   \vspace{-3mm}
   \label{tab:Benchmarks}
   \hspace*{-0.05\linewidth}
   \resizebox{1\linewidth}{!}{
      \begin{tabular}{|l|c|c|c|c|c|c|c|}
      \hline
      \textbf{Circuits} & \textbf{\# Objects} & \textbf{\# Standard} & \textbf{\# Movable} & \textbf{\# Fixed} & \textbf{\# Nets} & \textbf{\# Pins} & \textbf{Target}  \\ 
                        &                     & \textbf{cells}       & \textbf{macros}     & \textbf{macros}   &           
            &                  & \textbf{density} \\ \hline      
      ADAPTEC1  &   211,447 &   210,904 & 63    & 480    &   221,142 &   944,053  & 100\% \\ \hline
      ADAPTEC2  &   255,023 &   254,457 & 127   & 439    &   266,009 & 1,069,482  & 100\% \\ \hline
      ADAPTEC3  &   451,650 &   450,927 & 58    & 665    &   466,758 & 1,875,039  & 100\% \\ \hline
      ADAPTEC4  &   496,054 &   494,716 & 69    & 1,260  &   515,951 & 1,912,420  & 100\% \\ \hline
      BIGBLUE1  &   278,164 &   277,604 & 32    & 528    &   284,479 & 1,144,691  & 100\% \\ \hline
      BIGBLUE2  &   557,866 &   534,782 & 959   & 22,125 &   577,235 & 2,122,282  & 100\% \\ \hline
      BIGBLUE3  & 1,096,812 & 1,093,034 & 2,549 & 1,229  & 1,123,170 & 3,833,218  & 100\% \\ \hline
      BIGBLUE4  & 2,177,353 & 2,169,183 & 199   & 7,970  & 2,229,886 & 8,900,078  & 100\% \\ \hline
      ADAPTEC5  &   843,128 &   842,482 & 76    & 570    &   867,798 & 3,493,147  & 50\%  \\ \hline
      NEWBLUE1  &   330,474 &   330,073 & 64    & 337    &   338,901 & 1,244,342  & 80\%  \\ \hline
      NEWBLUE2  &   441,516 &   436,516 & 3,748 & 1,252  &   465,219 & 1,773,855  & 90\%  \\ \hline
      NEWBLUE3  &   494,011 &   482,833 & 51    & 11,127 &   552,199 & 1,929,892  & 80\%  \\ \hline
      NEWBLUE4  &   646,139 &   642,717 & 81    & 3,341  &   637,051 & 2,499,178  & 50\%  \\ \hline
      NEWBLUE5  & 1,233,058 & 1,228,177 & 91    & 4,790  & 1,284,251 & 4,957,843  & 50\%  \\ \hline
      NEWBLUE6  & 1,255,039 & 1,248,150 & 74    & 6,815  & 1,288,443 & 5,307,594  & 80\%  \\ \hline
      NEWBLUE7  & 2,507,954 & 2,481,372 & 161   & 26,421 & 2,636,820 & 10,104,920 & 80\%  \\ \hline
      \end{tabular}
   }
   \vspace{-2mm}
\end{table}
